Search for CPT Violation with the FOCUS Experiment and Measurement of $\Lambda_b$ lifetime in the decay $\Lambda_b\to J/\psi \Lambda$ with the D\O Experiment

We have performed a search for CPT violation in neutral charm meson oscillations using data from the FOCUS Experiment. While flavor mixing in the charm sector is predicted to be small by the Standard Model, it is still possible to investigate CPT violation through a study of the proper time dependence of a CPT asymmetry in right-sign decay rates for $D^0\to K^-\pi^+$ and $\d0b\to K^+\pi^-$. This asymmetry is related to the CPT violating complex parameter $\xi$ and the mixing parameters $x$ and $y$: $A_{CPT}\propto{\rm Re} \xi y-{\rm Im} \xi x$. Our 95% confidence level limit is $-0.0068<{\rm Re} \xi y-{\rm Im} \xi x<0.0234$. Within the framework of the Standard Model Extension incorporating general CPT violation, we also find 95% confidence level limits for the expressions involving coefficients of Lorentz violation. We present measurements of the \lb lifetime in the exclusive decay channel \lbdec with $J/\psi \to \mu^+ \mu^-$ and $\Lambda \to p \pi^-$, the $B^0$ lifetime in the decay \bddecks with $J/\psi \to mu^+ \mu^-$ and $K^0_{S} \to \pi^+ \pi^-$, and the ratio of these lifetimes. The analysis is based on approximately 225 pb$^{-1}$ of data recorded with the D{\O}detector in $p bar{p}$ collisions at $\sqrt{s} =1.96$ TeV. The \lb lifetime is determined to be $\tau(\Lambda^0_b) = 1.36 \pm 0.3 ps$, the $B^0$ lifetime $\tau(\Lambda^0_b) = 1.43 \pm 0.12 ps$, and the ratio $\fr ac{\tau(\Lambda_b)}{\tau(B_d)}=0.95\pm0.22$. In contrast with previous measurements using semileptonic decays, this is the first determination of the \lb lifetime based on a fully reconstructed decay channel.

==> abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
This dissertation describes two different projects from two different experiments.
We have performed a search for CPT violation in neutral charm meson
oscillations using data from the FOCUS Experiment.  
While flavor mixing in the charm sector is predicted to be 
small in the Standard Model, it is still possible to 
investigate CPT violation through a study
of the proper time dependence of a CPT asymmetry in
right-sign decay rates for $D^0\rightarrow K^-\pi^+$ and
$\d0b\rightarrow K^+\pi^-$. This asymmetry is related
to the CPT violating complex parameter $\xi$ and the
mixing parameters $x$ and $y$: $A_{CPT}\propto{\rm Re}\,\xi\,y-{\rm Im}\,\xi\,x$.
We determine a 95\% confidence level limit
of $-0.0068<{\rm Re}\,\xi\,y-{\rm Im}\,\xi\,x<0.0234$.
Within the framework of the Standard Model Extension incorporating general
CPT violation, we also find 95\% confidence level limits for the
expressions involving coefficients of Lorentz violation
 of 
$(-2.8<N(x,y,\delta)(\Delta a_0 + 0.6\,\Delta a_Z)<4.8)\times 10^{-16}$~GeV, $(-7.0<N(x,y,\delta)\Delta a_X<3.8)\times 10^{-16}$~GeV,
and $(-7.0<N(x,y,\delta)\Delta a_Y<3.8)\times 10^{-16}$~GeV, where
$N(x,y,\delta)$ is a normalization factor that incorporates mixing
parameters $x$, $y$ and the doubly Cabibbo suppressed to Cabibbo
favored relative strong phase $\delta$.


We also present measurements of the \lb\ lifetime in the exclusive decay channel 
\lbdec\, with $J/\psi \rightarrow \mu^+ \mu^-$ and
$\Lambda \rightarrow p \pi^-$, the $B^0$ lifetime in the decay \bddecks\ with $J/\psi \rightarrow \mu^+ \mu^-$ and
$K^0_{S} \rightarrow \pi^+ \pi^-$, and the ratio of these lifetimes.
The analysis is based on approximately 225 pb$^{-1}$ of data recorded with the D\O\ detector in $p\bar{p}$ collisions at $\sqrt{s} =1.96$~TeV. The \lb\ lifetime is determined to be $\tau(\Lambda^0_b) = 1.36 \pm 0.30 ~({\rm stat}) \pm 0.07({\rm syst})$~ps, the $B^0$ lifetime $\tau(B_d) = 1.43 \pm 0.12~({\rm stat})\pm 0.04~({\rm syst})$~ps, and the ratio $\frac{\tau(\Lambda_b)}{\tau(B_d)}=0.95 \pm 0.22 \pm 0.05$.\\
 In contrast with previous measurements using semileptonic decays, this is the first determination of the \lb\ lifetime based on a fully reconstructed decay channel.


==> acknowledge.tex <==
\noindent 
First of all, my deepest gratitude goes to my advisors, Dr. Rick Van Kooten and Dr. Rob Gardner.
Throughout the years of my Ph.D. study, they were always willing to mentor, 
encourage, and support me. Their  
expertise and enthusiasm in the field of high energy physics, 
as well as their unique insightful way of approaching problems, 
are among the most valuable resources for me.

%In particular I would like to point out Dr. Rob Gardner's insights into the computational challenges that lie ahead in the field of High Energy Physics. I would also like to point out Dr. Rick Van Kooten's insights and continually making different B physics topics interesting. 

I would like to thank Dr. Alan Kosteleck\'y for his explanations of the CPT and Lorentz Violation framework and also for his comments and suggestions during the process of publishing the CPT paper, which has been used in this thesis.   

I would like to thank Dr. Fred Luehring for his suggestions when I have been at crossroads in my career and his help with some computer software. Along the same lines I would like to thank Thom Sulanke for his help at solving a lot of technical questions.

I would like to thank people from the FOCUS Collaboration, in particular 
Jim Wiss, Gianluigi Boca, Topher Cowfield, John Link, Eric Vaandering, Kevin Stenson and Harry Cheung for their continual help with any question that I had, and also for their input on making the first part of this thesis possible. 

I would like to thank Indiana University D\O\ group, in particular 
Daria Zieminska and Andrzej Zieminski for the usuful disscussions and suggestions during our Indiana University D\O\ group meetings.

I would like to thank people from the B-Physics group at D\O\, in particular
Vivek Jain, Brad Abbott, Rick Jessik, Guenadi Borisov, Andrei Nomerotski, Sergey Burdin for their continual help with any question that I had, and also for their input on making the second part of this thesis possible. 

I would like to thank friends in the Physics Department, Maciej Swat, Prabudha Chakraboty, Jundong Huang and Chunhui Luo for the great physics discussions we have had and also for their friendship.

Finally I would like to thank my beautiful fianc\'ee Ilse Friberg and my parents Avni and Fatmire Kryemadhi for their encouragement and support in the process of making this thesis happen, they have been happy for my achievements and patient with my frustrations.    




==> dedication.tex <==
To God:
Who created so much beauty in the universe for us to study.\\

 ''The heavens declare the glory of God; 
 the skies proclaim the work of his hands''.\\ 
 \centerline {Psalm 19:1}

%To my beautiful fianc\e Ilse Friberg and my parents:\\ 
%``For their encouragement and support through ups and downs in writing this thesis''
 


==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \clearpage

\begin{thebibliography}{99} 

\def\NPB{{\it Nucl. Phys.} B}
\def\PLB{{\it Phys. Lett.}  B}
\def\PRL{\it Phys. Rev. Lett.}
\def\PRD{{\it Phys. Rev.} D}
\def\ZPC{{\it Z. Phys.} C}
\def\EPJ{{\it Eur. Phys. J.} C}
\def\NIA{{\it Nucl. Inst. and Meth.} A}
\def\CPC{\it Comput. Phys. Commun.}
\def\SNP{\it Sov.~J.~Nucl.~Phys.}
\def\NIMA{{\it Nucl. Instr. Methods Phys. Res.} A}
\def\NIM{{\it Nucl. Instr. Methods} A}
%\def\prl{Phys. Rev. Lett.}
%\def\prb{Phys. Rev. {\bf B}}
%\def\pre{Phys. Rev. {\bf E}}
%\def\PRD{Phys. Rev. D}
%\def\PLB{Phys. Lett. {\bf B}}
% A useful Journal macro
%\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}
% A useful Journal macro
\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}

%\bibitem{review-b-at-tevatron} ``$B$ Physics at the Tevatron: Run~II
%and Beyond'', Fermilab-Pub-01/197 (2001).
%hep-ph/0201071

%\bibitem{review-cern-2002} ``The CKM Matrix and the Unitarity Triangle'',
%Proceedings of the First Workshop on the CKM Unitarity Triangle, 
%CERN, February 2002.
%hep-ph/0304132

%\bibitem{thesis:murphy} 
%C.~Murphy, Indiana University, PhD dissertation, ``Inclusive $J/\psi$ Production at \D0'' (1995).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ch1b: Theory of CPT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{weinberg} S.~Weinberg,
\Journal{\PRL}{19}{1264}{1967}.

\bibitem{neutrino} {\it Atmospheric Neutrino Results From Super Kamiokande and Kamiokande; Evidence of Neutrino Oscillations.}, {\it Nucl.~Phys.~Proc.~Suppl.} {\bf 77}, 123 (1999). 

\bibitem{breadbutter} Zoltan Kunszt,
``Bread and Butter standard model'', hep-ph/0004103.

\bibitem{electroweak} 
Ch.~Quigg, {\it The Electroweak Theory}, hep-ph/0204104. 

\bibitem{kostelecky-95} V.A. Kosteleck\'y, R. Potting,
\Journal{\PRD}{51}{3923}{1995}.
%\PRD{\bf 51} 3923 (1995).

\bibitem{kostelecky} V.A. Kosteleck\'y,
\Journal{\PRD}{64}{076001}{2001}. {\it Section 2 of the paper gives relationships between formalisms}.
%\PRD{\bf 64} 076001 (2001).

\bibitem{alanbook}
V.~A.~Kosteleck\'y, 
 {\it CPT and Lorentz Symmetry II}; 
 Singapore, World Scientific Publishing Co.~Pte.~Ltd. (2002).

\bibitem{kostelecky99} V.A. Kosteleck\'y,
\Journal{\PRD}{61}{016002}{1999}.
%\PRD{\bf 61} 016002 (1999).
%{\it Section 2 of the paper gives relationships between formalisms}.

\bibitem{ktev} Y.B. Hsiung for the KTeV Collaboration,
Proc.\ QCD Euroconference 99, Montpellier, France, July 7-13, 1999.  Also
available as FERMILAB-Conf-99/338-E (KTeV).

\bibitem{ktevlv}
H.~Nguyen, 
{\it CPT results from KTeV}, hep-ex/{\rm 0112046}.

\bibitem{opal} OPAL Collaboration (K. Ackerstaff {\it et al.}),
\Journal{\ZPC}{76}{401}{1997}.
%Z.~Phys.~C{\bf 76}: 401-415, 1997. 

\bibitem{belle} Belle Collaboration (K. Abe, {\it et al.}),
\Journal{\PRL}{86}{3228}{2001}.
%\PRL{\bf 86}, 3228 (2001). 

\bibitem{focusycp} FOCUS Collaboration (J. Link {\em et al.}),
\Journal{\PLB}{485}{62}{2000}.
%\PLB{\bf 485}, 62 (2000).

\bibitem{belleycp} Belle Collaboration (K.~Abe {\em et al.}),
\Journal{\PRL}{88}{162001}{2002}.
%\PRL{\bf 88}, 162001 (2002).

\bibitem{babary} BaBar Collaboration (B.~Aubert {\em et al.}),
{\it Search for a Lifetime Difference in $D^0$ Decays}, hep-ex/{\rm 0109008}.

\bibitem{cleo}CLEO Collaboration (R. Godang {\em et al.}),
\Journal{\PRL}{84}{5038}{2000}.
%\PRL{\bf 84}, 5038 (2000).

\bibitem{linkrd}FOCUS Collaboration (J. Link {\em et al.}),
\Journal{\PRL}{86}{2955}{2001}.
%\PRL{\bf 86}, 2955 (2001).


%\bibitem{pdg}Review of Particle Properties,  D.E. Groom {\em et al.}, 
%\Journal{\EPJ}{15}{1}{2000}.


%\bibitem{e687}E687 Collaboration P.L. Frabetti {\em et al.}, 
%\Journal{\PLB}{370}{222}{1996}.

\bibitem{ref:abaz} FOCUS Collaboration (J. Link {\em et al.}),
\Journal{\PLB}{556}{7}{2003}.
%\PLB{\bf 556}, 7 (2003).

\bibitem{colladay-kostelecky} D. Colladay and V.A. Kosteleck\'y,
\Journal{\PRD}{55}{67600}{1997};
%\PRD{\bf 55} 67600 (1997);
\Journal{\PRD}{58}{116002}{1998};
%\PRD{\bf 58} 116002 (1998).
 V.A. Kosteleck\'y,
\Journal{\PRD}{69}{105009}{2004}.

\bibitem{kostelecky-prl} V.A. Kosteleck\'y,
\Journal{\PRL}{80}{1818}{1998}.
%\PRL{\bf 80}, 1818 (1998).

\bibitem{JeanMeeus} Jean Meeus,
Astronomical Algorithms First English Edition (1991).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ch2: FOCUS Detector
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{expE687}
  E687 Collaboration (P.L.Frabetti {\it et al}), 
\Journal{\NIA}{320}{519}{1992}.
%Nuclear Instruments and Methods A, {\bf 320}, 519 (1992).

\bibitem{E831beam}
P. Kasper, R. Currier, P. Garbincius, and J. Butler, Wide band to double band upgrade. Technical Report TM-1552, Fermilab, 1988.

\bibitem{E831ks}
FOCUS Collaboration (J. M. Link {\it et al.}), 
\Journal{\NIA}{484}{174}{2002}.
%Nuclear Instruments and Methods A, {\bf 484}, 174  (2002). 

\bibitem{EricThesis}
E. Vaandering, Ph.D. thesis, University of Colorado, Boulder, January 2000.

\bibitem{LinkThesis}
J. M. Link, Ph.D. thesis, University of California, Davis, March 2001.

\bibitem{E831tsil}
J. M. Link {\it et al.}, 
\Journal{\NIA}{516}{364}{2004}.
%Target Silicon, hep-ex/{\rm 0204023}, 2002.

\bibitem{E831id}
FOCUS Collaboration (J. M. Link {\it et al.}),
\Journal{\NIA}{484}{270}{2002}.
% Nuclear Instruments and Methods A, {\bf 484}, 270  (2002).  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%ch2b Data Analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\bibitem{pdg2000}Review of Particle Properties,  D.E. Groom {\em et al.}, 
%\EPJ{\bf 15} 1 (2000).

\bibitem{pdg2004}Review of Particle Properties,  S.~Eidelman {\em et al.}, 
\Journal{\PLB}{592}{1}{2004}.
%\PLB{\bf 592}, 1 (2004).


\bibitem{e687}E687 Collaboration (P.L. Frabetti {\em et al.}), 
\Journal{\PLB}{370}{222}{1996}.
%\PLB{\bf 370}, 222 (1996).

\bibitem{pythia61} T.~Sj\"{o}strand {\it et al.}, 
\Journal{\CPC}{135}{238}{2001}.
%Comput.\ Phys.\ Commun., {\bf 135}, 238 (2001).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%ch2c_lbintro
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{UA1lb}
C.~Albajar {\it et al.}, 
%{\it First Observation of the Beauty Baryon \lb\ in the decay channel \lbdec\ at the CERN proton-antriproton collider},
\Journal{\PRD}{273}{540}{1991}.
%\PRD{\bf 273}, 540 (1991).

\bibitem{alephlb}
 ALEPH Collaboration (D.~Buskulic {\it et al.}), 
%Measurement of the Mass of the $\Lambda_b$ Baryon, 
\Journal{\PLB}{380}{442}{1996}.
%\PLB{\bf 380}, 442 (1996).

\bibitem{delphilb}
 DELPHI Collaboration (P.~Abreu {\it et al.}), 
%Search for Exclusive Decays of $\Lambda_b$ Baryon and Measurement of its Mass, 
\Journal{\PLB}{374}{351}{1996}.
%\PLB{\bf 374}, 351 (1996). 

\bibitem{cdflb}
 CDF Collaboration (F.~Abe {\it et al.}), 
%Observation of $\Lambda_b\rightarrow J/\psi \Lambda$ at the Fermilab Proton-Antiproton Collider, 
\Journal{\PRD}{55}{1142}{1997}.
%\PRD{\bf 55}, 1142 (1997).

\bibitem{eduardo}
D\O\ Collaboration (V~.M.~Abazov {\it et al.}), 
 {\it Measurement of \lb\ lifetime in the decay \lbdec\ with D\O\ detector}, hep-ex/0410054.
Submitted to {\it Phys.~Rev.~Lett.}.
% (Submitted to \Journal{\PRL}) 
%\bibitem{PDGlb} Particle Data Group (see webpage http://pdg.lbl.gov).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ch2d_lbtheory 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\bibitem{Vcd}
G.~Kane, Modern Elementary Particle Physics, Addision-Wesley, 1993

%\bibitem{RatioResults1}
%S.~Eidelman {\it et al.}, \Journal{\PLB}{592}{1}{2004}; E.~Barberio, presented at the Workshop on the CKM Unitary Triangle, http://ckm-workshop.web.cern.ch; M.~Battaglia {\it et al.}, hep-ph/0304132.

%\bibitem{RatioResults2}
%LEP B Lifetime Working Group, http://lepbosc.web.cern.ch/LEPBOSC/lifetimes/lepblife.html.

\bibitem{qcdprediction}
M.~Ciuchini, E.~Franco, V.~Lubicz and F.~Mescia,~\Journal{\NPB}{625}{211}{2002}; E.~Franco, V.~Lubicz, F.~Mescia and C.~Tarantino,~\Journal{\NPB}{633}{212}{2002}.

\bibitem{1mbcorrection}
F.~Gabbiani, A.~I.~Onishchencko and A.~A.~Petrov, 
\Journal{\PRD}{68}{114006}{2003}
%Phys.~Rev.~D {\bf 68}, 114006 (2003).

\bibitem{fabrizio2}
F.~Gabbiani, A.~I.~Onishchencko and A.~A.~Petrov,
{\it Spectator Effects and Lifetimes of Heavy Hadrons}, hep-ph/0407004. 

\bibitem{newratiotheory}  C.~Tarantino, 
\Journal{\EPJ}{33}{895}{2004}.


\bibitem{bigi}
I.~Bigi {\it et al.}, hep-ph/0001003, hep-ph/9401298; M.~B.~Voloshin, hep-ph/0004257.

\bibitem{neubert}
M.~B.~Voloshin, Phys.~Rep.~{\bf 320}, 275 (1999); B.~Guberina, B.~Melic, and H.~Stefancic, \Journal{\PLB}{469}{253}{1999}; 
M.~Neubert and C.~T.~Sachrajda, \Journal{\NPB}{483}{339}{1997}.

\bibitem{shifman}
M.~A.~Shifman and M.~B.~Voloshin, \Journal{\SNP}{41}{120}{1985}.

\bibitem{guberina}
B.~Guberina {\it et al.}, \Journal{\PLB}{89}{111}{1979}; N.~Bilic {\it et al.}, \Journal{\NPB}{248}{261}{1984}; B.~Guberina {\it et al.}, \Journal{\ZPC}{33}{297}{1986}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{comment}

%\bibitem{PDG} Particle Data Group (see webpage http://pdg.lbl.gov).

\bibitem{physics:cdfd0} T.~LeCompte, H.~T.~Diehl, ``The CDF and \D0 Upgrades for Run~II";
Fermilab Annual Review (2000).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The D0 Detector
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{holmes} S.~D.~Holmes, 
%``Design Criteria and Performance Goals for the
%Fermilab Main Injector'',
 {\it Part. Accel.} {\bf 58}, 39 (1997), Fermilab-Conf-97/038.
%The Run II Handbook,
%http://www-bd.fnal.gov/lug/runll\_handbook/Runll\_index.html, (1995)

\bibitem{recycler} G.~P.~Jackson, 
``The Fermilab Recycler Ring Technical
Design Report'',
 Fermilab-TM-1991 (1996).

\bibitem{d0tdwhatever} D\O \ Collaboration (S.~Abachi {\it et al.}),
``The D\O \ Upgrade: Detector and its Physics'',
Fermilab-Pub-96/357-E (1996); ``The D\O \ Upgrade Forward Preshower,
Muon System, and Level~2 Trigger'', Fermilab-FN-639 (1996).


\bibitem{d0runI} D\O \ Collaboration (S.~Abachi {\it et al.}),
\Journal{\NIMA}{338}{185}{1994}.
% Nucl. Instr. Methods Phys. Res. A {\bf 338}, 185 (1994).

% Silicon
\bibitem{lipton} R.~Lipton for the D\O \ Collaboration,
\Journal{\NIM}{418}{85}{1998}.
% Nucl. Instr. Meth. {\bf A418}, 85 (1998).
\bibitem{FNALTM1892} R.~Yarema {\sl et al.}, 
``A beginners Guide to the SVX~II~Chip'',
 Fermilab-TM-1892 (1994).

% Out tracker
\bibitem{wayne} M.~Wayne for the D\O \ Collaboration,
\Journal{\NIM}{408}{103}{1998}.
% Nucl. Instr. Meth. {\bf A408},103 (1998).

\bibitem{cdf-svx3} T.~Zimmermann {\it et al.},
%``SVX3: A Deadtimeless Readout Chip for Silicon Strip Detectors'',
%%Proceedings of Frontier Detectors for Frontier Physics: 7th Pisa Meeting
%%on Advanced Detectors, La Biodola, Isola d'Elba, Italy, May 25-31, 1997},
\Journal{\NIMA}{409}{1}{1998}.
%Nucl. Instr. Methods Phys. Res., {\bf A409}, 1 (1998); FERMILAB-Conf-97/427.

%Muon
\bibitem{d0scintnim} B.~S.~Acharya {\it et al}, 
%``Scintillation Counters for the D\O \ Upgrade'', 
\Journal{\NIM}{401}{45}{1997}.
%Nucl. Instr. Meth. {\bf A401}, 45 (1997).

\bibitem{abramov} V.~Abramov {\sl it al.}, 
%``Forward muon system for the D\O \ Upgrade'', 
\Journal{\NIM}{419}{660}{1998}.
%Nucl. Instr. Meth. {\bf A419}, 660 (1998).

\bibitem{eroshin}
O.~Eroshin, D.~Denisov, ``Status of forward muon reconstruction program'', \D0 Note 3714 (1999).

\bibitem{d0daq}
\D0 Collaboration ``The \D0 Upgrade", \D0 internal technical documentation (1995).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ch3b: Lb Analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{AATrack} 
\begin{verbatim}
http://d0server1.fnal.gov/users/nomerot/Run2A/BANA/Dskim.html.
\end{verbatim}

\bibitem{primary}
DELPHI Collaboration (J.~Abdallah {\it et al.}),
\Journal{\EPJ}{32}{184}{2004}.
% Eur.\ Phys.\ J. {\bf C32} (2004) 184.

\bibitem{bana} 
\begin{verbatim}
http://d0server1.fnal.gov/users/nomerot/Run2A/BANA.html .
\end{verbatim}


\bibitem{evtgen} A. Ryd, D. Lange, {http://www.slac.stanford.edu/$\sim$lange/EvtGen/ . }

%\bibitem{qq} QQ - the CLEO event generator, {http://www.lns.cornell.edu/public/CLEO/soft/QQ}

\bibitem{pythia} H.~U.~Bengtsson and T.~Sjostrand,
\Journal{\CPC}{46}{43}{1987}.
%                 Comp. Phys. Comm. {\bf 46}, 43 (1987).

%\bibitem{CDF_bs00} F.~Abe {\it et al.}, CDF Collaboration 
%              Phys. Rev. Lett., {\bf xx}, xxxx (2000).

%\bibitem{CDF_bs96} F.~Abe {\it et al.}, CDF Collaboration 
%              Phys. Rev. Lett., {\bf 77}, 1945 (1996).
\bibitem{d0mess}
\begin{verbatim}
http://www-d0.fnal.gov/computing/MonteCarlo/generator_tools/d0_mess.html.
\end{verbatim}

\bibitem{geant}
\begin{verbatim}
http://wwwasdoc.web.cern.ch/wwwasdoc/pdfdir/geant.pdf.
\end{verbatim}

\bibitem{leptonp_lambdab}
Abaz Kryemadhi, Rick Van Kooten,
{\sl A Measurement of the $\Lambda_b^0$ Baryon 
Lifetime Using the
$ \Lambda_b^0 \rightarrow  J/\psi \Lambda$ Decay Mode},
\D0\ Note 4232, 15 Aug. 2003.

\bibitem{leptonp_lambdab_update}
Abaz Kryemadhi, Rick Van Kooten,
{\sl (Re)Establishing the $\Lambda_b^0$ signal via the
$ \Lambda_b^0 \rightarrow  J/\psi \Lambda$ Decay Mode},
\D0\ Note 4355, 23 Feb. 2004.

\bibitem{daria_lambdab}
Daria Zieminska,
{\sl Do We Understand the $\Lambda_b$ Signal?}, 
\D0\ Note 4269, 1 Oct. 2003.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ch4: The D0 Software, changed?
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{bs:chunhui_fit}
Chunhui Luo, Ph.D. thesis, Indiana University, Bloomington, July 2003. 
%\verb"http://hep.physics.indiana.edu/~chuluo/BsJpsiPhi/lifetime".


\end{thebibliography} 


